A Corpus for Reasoning About Natural Language Grounded in Photographs

We introduce a new dataset for joint reasoning about natural language and images, with a focus on semantic diversity, compositionality, and visual reasoning challenges. The data contains 107,292 examples of English sentences paired with web photographs. The task is to determine whether a natural language caption is true about a pair of photographs. We crowdsource the data using sets of visually rich images and a compare-and-contrast task to elicit linguistically diverse language. Qualitative analysis shows the data requires compositional joint reasoning, including about quantities, comparisons, and relations. Evaluation using state-of-the-art visual reasoning methods shows the data presents a strong challenge.

==> separate_sup.tex <==
%
%


\input{header}
\externaldocument{rnlvr}
\author{Alane Suhr\affilone\thanks{\hspace{5pt}Contributed equally.},\hspace{1pt} Stephanie Zhou\thanks{\hspace{5pt}Work done as an undergraduate at Cornell University.}\hspace{4pt},\hspace{-3pt}\footnotemark[1] \hspace{3.5pt}Ally Zhang\affilone, Iris Zhang\affilone, Huajun Bai\affilone, {\normalfont and} Yoav Artzi\affilone
\vspace{0.5em}\\
 \affilone Cornell University  Department of Computer Science and Cornell Tech \\ %
  New York, NY 10044 \\
  {\tt \{suhr, yoav\}@cs.cornell.edu \hspace{1em}\{az346, wz337, hb364\}@cornell.edu}
  \vspace{0.5em}\\
   $^\dagger$University of Maryland Department of Computer Science\\
 College Park, MD 20742 \\
  {\tt stezhou@cs.umd.edu}}
  
\date{}

\title{A Corpus for Reasoning About Natural Language \\ Grounded in Photographs \\ (Appendix)}


\begin{document}
\maketitle

\setcounter{figure}{3}
\setcounter{table}{6}
\appendix
\input{supplementary}

\clearpage
\balance
\bibliography{main}
\bibliographystyle{acl_natbib}


\end{document}
